Implicit Neural Representations for Image Compression

Recently Implicit Neural Representations (INRs) gained attention as a novel and effective representation for various data types. Thus far, prior work mostly focused on optimizing their reconstruction performance. This work investigates INRs from a novel perspective, i.e., as a tool for image compression. To this end, we propose the first comprehensive compression pipeline based on INRs including quantization, quantization-aware retraining and entropy coding. Encoding with INRs, i.e. overfitting to a data sample, is typically orders of magnitude slower. To mitigate this drawback, we leverage meta-learned initializations based on MAML to reach the encoding in fewer gradient updates which also generally improves rate-distortion performance of INRs. We find that our approach to source compression with INRs vastly outperforms similar prior work, is competitive with common compression algorithms designed specifically for images and closes the gap to state-of-the-art learned approaches based on Rate-Distortion Autoencoders. Moreover, we provide an extensive ablation study on the importance of individual components of our method which we hope facilitates future research on this novel approach to image compression.

==> img/kodak_div_tikz.tex <==
% This file was created with tikzplotlib v0.9.15.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.75,0.75,0}
\definecolor{color1}{rgb}{0,0.75,0.75}
\definecolor{color2}{rgb}{1,0.549019607843137,0}
\definecolor{color3}{rgb}{1,0,1}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.04,0.5)},
  anchor=west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Bitrate [bpp]},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={PSNR [dB]},
ymin=22, ymax=38,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
0.173088073730469 21.4476394664869
0.173194885253906 21.4495500790818
0.181832207573785 21.6531880117728
0.200492858886719 22.7689153888408
0.221154106987847 23.8142136843025
0.242518954806858 24.6513804053415
0.263965182834201 25.2982514469326
0.284738328721788 25.7993763811811
0.306045532226562 26.1862731698452
0.326588948567708 26.6111550128765
0.346971299913194 26.9458129308626
0.366207546657986 27.2652442529704
0.386786566840278 27.5856274082302
0.404252794053819 27.8162650363736
0.42309824625651 28.0766660430844
0.441468980577257 28.2998995525742
0.459219190809462 28.5316776148752
0.477264404296875 28.736250715126
0.492713928222656 28.8902962471962
0.508269415961372 29.0763645351773
0.525771247016059 29.2552481039273
0.541648864746094 29.3925190395401
0.55777825249566 29.5418087430924
0.573367648654514 29.6916637216744
0.587676154242622 29.8186501575044
0.602671305338542 29.9402346364983
0.617232428656684 30.0842202831602
0.633494906955295 30.1979305110498
0.645818922254774 30.3055793003623
0.65979258219401 30.4123444396366
0.67313469780816 30.5169676529513
0.686729431152344 30.6201459607619
0.70225101047092 30.7339874688377
0.711793687608507 30.824602513179
0.728571573893229 30.9369707601915
0.74310302734375 31.0337528508283
0.751000298394097 31.0971346381735
0.767808702256944 31.198740701572
0.77903323703342 31.2713729978675
0.785571628146701 31.3433831166696
0.804250081380208 31.4590582031314
0.813478257921007 31.5069243731609
0.823445638020833 31.5789216862731
0.840131123860677 31.6920530707512
0.849210951063368 31.7400265151381
0.86468760172526 31.8413732396478
0.871844821506076 31.8975091404033
0.883314344618056 31.9445681799395
0.901442633734809 32.0522731109099
0.905520968967014 32.0938691876654
0.909598456488715 32.1357702757408
0.929573059082031 32.2427914116632
0.942776150173611 32.2971270394421
0.951766120062934 32.3634411671708
0.963646782769097 32.4329262653617
0.978990342881944 32.5093902926715
0.99466790093316 32.5876370407966
1.01253679063585 32.6748406247428
1.02317555745443 32.7358441016835
1.03658548990885 32.820837433924
1.05658213297526 32.9139921106937
1.06909518771701 32.9896266260409
1.0910898844401 33.0871829729445
1.10433790418837 33.1723219251647
1.12647840711806 33.2650809704275
1.14399549696181 33.3717133874192
1.16216193305122 33.4833986413856
1.18948109944661 33.5902855850298
1.2094243367513 33.6916280023872
1.23875766330295 33.8234536944109
1.26397196451823 33.9499351854135
1.28432973225911 34.0567005167935
1.31484985351562 34.174299165228
1.35758293999566 34.3411026969898
1.36760033501519 34.4242453174152
1.40113152398003 34.5988464563854
1.45262400309245 34.7890147979419
1.49368540445964 34.9222123098614
1.52523634168837 35.0707509483601
1.57024298773872 35.2672310396225
1.62787712944878 35.4769188963088
1.67370012071398 35.6678532513435
1.74298519558377 35.8791631063342
1.79922061496311 36.1050881938395
1.8565190633138 36.3510343448622
1.94589657253689 36.6207985293453
2.01052093505859 36.8825673575392
2.12093777126736 37.2141668918593
2.20443216959635 37.5279266196196
2.34632280137804 37.9180029349037
2.46919335259332 38.3103533005481
2.59428914388021 38.7464462097178
2.8139894273546 39.2558654521095
3.08015950520833 39.850845643849
3.39191691080729 40.4951052340247
3.81007639567057 41.3316757055248
4.28460947672526 42.2390347531526
4.87249162462023 43.3501344967227
5.96051873101128 44.5690974432578
};
\addlegendentry{JPEG Matlab}
\addplot [semithick, black]
table {%
2.39732276068793 39.7920009903891
1.19824049207899 35.6807191218559
0.798279656304254 33.4899612266554
0.598828633626302 32.0897400948338
0.47928958468967 31.0745756380738
0.398624844021267 30.3007693809278
0.341842651367188 29.6961166732528
0.298562791612413 29.191735537599
0.265726725260417 28.7742265146691
0.239408704969618 28.4165903036621
0.217565748426649 28.0992240331438
0.199173821343316 27.7966358468974
0.184435526529948 27.5544696237349
0.17067379421658 27.3169933644787
0.159484015570747 27.1182506401724
0.14888424343533 26.9228460066158
0.140762329101562 26.7574244386992
0.132455613878038 26.5862349961256
0.125798543294271 26.4403826660524
};
\addlegendentry{JPEG2000 CompressAI}
\addplot [semithick, color1]
table {%
1.17803192138672 38.2590314026528
1.05873023139106 37.573110745425
0.954195658365885 36.9268194278595
0.855121188693576 36.2731804223418
0.763151380750868 35.5948189090454
0.681227789984809 34.9556713070246
0.602615356445312 34.2940735357481
0.528513590494792 33.6236347665041
0.465172661675347 32.9876217730078
0.406661987304688 32.3674413657179
0.35382080078125 31.7413611914467
0.308003743489583 31.148308814915
0.264901902940538 30.5536551253969
0.226881239149306 29.9617217038047
0.193940056694878 29.4044957752005
0.165530734592014 28.8695561191948
0.14007568359375 28.3319094598586
0.119210984971788 27.8356649636595
0.100255330403646 27.3304621811179
0.0841759575737847 26.8469065562654
0.0704438951280382 26.3736301333705
0.0588616265190972 25.9240447126546
0.0493011474609375 25.4725996281505
0.041182623969184 25.0366805407434
0.0342814127604167 24.6144848301033
0.0285398695203993 24.2000466571302
0.0238571166992188 23.8178541080361
};
\addlegendentry{BPG}
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
0.0833536783854167 26.0485477551573
0.0833646986219618 25.9629581603874
0.154680040147569 27.4294359010241
0.251265631781684 28.6331865406372
0.252161661783854 28.6646300236762
0.866822984483507 32.3985409873846
};
\addlegendentry{Meta-learned SIREN (7 bit)}
\addplot [semithick, red, mark=*, mark size=3, mark options={solid}]
table {%
0.0712627834743924 24.7651702780793
0.139356825086806 26.200804918985
0.228336758083767 27.4498005956842
0.764495849609375 31.249215302645
};
\addlegendentry{SIREN (7 bit)}
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
0.036854138088706 22.3917525773196
0.073068129858253 23.1649484536082
0.15976223136717 24.639175257732
0.306812985825331 26.4123711340206
0.610059442158208 28.4020618556701
0.995244627343393 29.8659793814433
};
\addlegendentry{COIN}
\addplot [semithick, green!50!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0.131293402777778 27.5815367933339
0.208892822265625 29.1966941213848
0.319858127170139 30.9721687054992
0.478356255425347 32.8381911170407
0.66868421766493 34.5262427611008
0.93882581922743 36.7433646176229
1.25917222764757 38.5838558444321
1.66022406684028 40.5568737001521
};
\addlegendentry{Balle Hyperprior [2018]}
\addplot [semithick, color2, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0.122623019748264 26.9087869937475
0.188527425130208 28.2179270136604
0.287807888454861 29.6169118573908
0.440378824869792 31.277098217644
0.64813232421875 32.9561337034905
0.966976589626736 35.3809504728754
1.35116238064236 37.3969350820545
1.83327229817708 39.6213054445271
};
\addlegendentry{Balle Factorized [2018]}
\addplot [semithick, white!66.2745098039216!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0.119598388671875 28.5823153462971
0.183803982204861 29.9684631443886
0.270952012803819 31.3426011951914
0.417385525173611 33.3896634510393
0.594455295138889 35.1180880740638
0.805728488498264 36.7044737184614
};
\addlegendentry{Cheng Anchor [2020]}
\addplot [semithick, color3, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0.115576850043403 28.4310225629413
0.174492730034722 29.7674659602663
0.269036187065972 31.3214427460843
0.426951090494792 33.3629721212383
0.595265706380208 34.9492983081221
0.805914984809028 36.6223475379347
};
\addlegendentry{Cheng Attention [2020]}
\addplot [semithick, color0, dashed, mark=*, mark size=3, mark options={solid}]
table {%
0.0983615451388889 27.8943027478587
0.133877224392361 28.9573342584169
0.163170708550347 29.7151073176142
0.292575412326389 31.9194708448622
0.451419406467014 33.945835166573
0.650787353515625 35.8398544469014
0.790991889105903 36.9078287301004
1.06111992730035 38.4707221097341
};
\addlegendentry{Xie [2021]}
\end{axis}

\end{tikzpicture}


==> img/methodoverview.tex <==
\usetikzlibrary{shapes,arrows,positioning,calc,chains,scopes}

% colors
\definecolor{snowymint}{HTML}{E3F8D1}
\definecolor{wepeep}{HTML}{FAD2D2}
\definecolor{portafino}{HTML}{F5EE9D}
\definecolor{plum}{HTML}{DCACEF}
\definecolor{sail}{HTML}{A3CEEE}
\definecolor{highland}{HTML}{6D885A}
\definecolor{red}{HTML}{DE1616}
\definecolor{blue}{HTML}{4438F2}
\definecolor{green}{HTML}{35bf22}

\tikzstyle{signal}=[arrows={-latex},draw=black,line width=1pt,rounded corners=4pt]

% RNN
\tikzstyle{block}=[draw=black,line width=1.0pt]
\tikzstyle{cell}=[style=block,draw=highland,fill=snowymint,
    rounded corners]
\tikzstyle{celllayer}=[style=block,draw,fill=portafino,
    inner sep=1pt,outer sep=0,
    minimum width=28pt, minimum height=14pt]
\tikzstyle{pointwise}=[style=block,ellipse,fill=wepeep,
    inner sep=1pt,outer sep=0, minimum size=12pt]

\def\iolen{24pt}
\def\intergape{2pt}

% MLP and CNN
\tikzstyle{netnode}=[circle, inner sep=0pt, text width=20pt, align=center, line width=1.0pt]
\tikzstyle{inputnode}=[netnode, text width=24pt, fill=sail,draw=black]
\tikzstyle{hiddennode}=[netnode, fill=snowymint,draw=black]
\tikzstyle{outputnode}=[netnode, fill=plum,draw=black]

% Architecture
\def\layerwidth{90pt}
\def\layerheight{14pt}

\tikzstyle{layer}=[style=block, draw, fill=black!20!white,
    inner sep=1pt,outer sep=0, font=\footnotesize,
    text centered, 
    minimum width=\layerwidth, minimum height=\layerheight]

\tikzstyle{fc}=[style=layer, fill=blue!30!white]
\tikzstyle{conv}=[style=layer, fill=green!30!white]
\tikzstyle{activation}=[style=layer, fill=orange!30!white]
\tikzstyle{pool}=[style=layer, fill=red!30!white]
\tikzstyle{bn}=[style=layer, fill=cyan!30!white]
\tikzstyle{recurrent}=[style=layer, fill=purple!30!white]
\tikzstyle{softmax}=[style=layer, fill=yellow!30!white]
\tikzstyle{point}=[]
\tikzstyle{branch}=[coordinate]

\def\vlayerwidth{30pt}
\def\vlayerheight{3pt}
\def\vblockheight{28pt}

\tikzstyle{vlayer}=[minimum width=\vlayerwidth, minimum height=\vlayerheight]
\tikzstyle{vblock}=[minimum width=\vlayerwidth, minimum height=\vblockheight, text width=1cm, align=center]


% Precision, Recall
\colorlet{fn}{gray!90!green!30!white}
\colorlet{tp}{green!40!white}
\colorlet{fp}{red!40!white}
\colorlet{tn}{gray!90!red!20!white}

\begin{tikzpicture}[]
    \def\nodedist{25pt}
    \def\layerdist{80pt}
    \def\pindist{20pt}
    
    \tikzstyle{every pin edge}=[signal]
    \tikzstyle{annot} = [text width=4em, text centered]
    
    \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:$p_x$}] 
            (I1) at (0,-1.25*\nodedist) {$\gamma( p_x)$}; 
    \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:$ p_y$}] 
            (I2) at (0,-2.75*\nodedist) {$\gamma (p_y)$}; 
    % \foreach \y in {1,2}
    %     \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:Input \y}] 
    %         (I\y) at (0,-\y*\nodedist) {$p_x$};  
    
    \foreach \y in {1,...,4}
        \node[hiddennode] 
            (H\y) at ($(\layerdist,-\y*\nodedist) +(0, 0.5*\nodedist)$) {};
    \foreach \y in {1,...,4}
        \node[hiddennode] 
            (B\y) at ($(2*\layerdist,-\y*\nodedist) +(0, 0.5*\nodedist)$) {};
            
    \node[netnode,fill=red]
            (O1) at ($(3*\layerdist,-1*\nodedist)$) {$R$};
    \node[netnode,fill=green]
            (O2) at ($(3*\layerdist,-2*\nodedist)$) {$G$};
    \node[netnode,fill=blue]
            (O3) at ($(3*\layerdist,-3*\nodedist)$) {$B$};
    %\node (myfirstpic) at ($(4*\layerdist,-2*\nodedist)$){\includegraphics{kodim21.png}}
    %\node (myfirstpic) at ($(4*\layerdist,-2*\nodedist)$){ 
    %      \includegraphics{modelv3_bw7_adaround_iter_1000_adaround_reg_0.0001_retrain_epochs300_retrain_lr1e-06_bpp0.08296712239583333_psnr24.43883332554804.png}}
    \foreach \dest in {1,...,4}
        \foreach \source in {1,...,2}
            \draw[signal] (I\source) -- (H\dest);
    \foreach \dest in {1,...,4}
        \foreach \source in {1,...,4}
            \draw[signal] (H\source) -- (B\dest);
    \foreach \dest in {1,...,3}
        \foreach \source in {1,...,4}
            \draw[signal] (B\source) edge (O\dest);
            
    \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 2.5*\nodedist] (r1) at (0.5*\layerdist,-2*\nodedist) {};
    
    \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 3.5*\nodedist] (r2) at (1.5*\layerdist,-2*\nodedist) {};
    
    \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 3*\nodedist] (r3) at (2.5*\layerdist,-2*\nodedist) {};
    
    \node[rectangle,
    draw = black,
    text = black,
    minimum width = 0.5cm,
    minimum height = 0.5cm] (theta) at (1.5*\layerdist,-4.5*\nodedist){$\theta$};
    
    \foreach \source in {1,3}
        \draw[signal] (r\source) |- (theta);
    \draw[signal] (r2) -- (theta);
    
    \node[rectangle,
    draw = black,
    text = black,
    minimum width = 0.5cm,
    minimum height = 0.5cm] (dtheta) at (2*\layerdist,-5.5*\nodedist){$\Delta\theta$};
    
    \node[netnode,
    draw = black,
    text = black,
    text width=16pt] (minus) at (1.5*\layerdist,-5.5*\nodedist){$-$};
    \draw[signal] (theta) -- (minus);
    \draw[signal] (minus) -- (dtheta);
    
        \node[rectangle,
    align=center,
    draw = white,
    text = black,
    fill = portafino,
    minimum width = 3cm,
    minimum height = 1cm] (meta) at (0,-6.25*\nodedist) {Meta-learned Initialization \\  $\theta_0$};
    \draw[signal] (meta) |- (minus);
    
    \node[rounded corners=5pt,
    draw = black,
    text = black,
    minimum width = 2cm,
    minimum height = 1cm] (compress) at (3*\layerdist,-5.5*\nodedist){compress};
    \draw[signal] (dtheta) -- (compress);
    
    \node[rounded corners=5pt,
    draw = black,
    text = black,
    minimum width = 2cm,
    minimum height = 1cm] (decompress) at (3*\layerdist,-7*\nodedist){decompress};
    
    
    \node[rectangle,
    draw = black,
    text = black,
    minimum width = 0.5cm,
    minimum height = 0.5cm] (dthetatilde) at (2*\layerdist,-7*\nodedist){$\Delta \Tilde{\theta}$};
    \draw[signal] (decompress) -- (dthetatilde);
    
    \node[netnode,
    draw = black,
    text = black,
    text width=16pt] (plus) at (1.5*\layerdist,-7*\nodedist){$+$};
    \draw[signal] (dthetatilde) -- (plus);
    \draw[signal] (meta) |- (plus);
        \node[rectangle,
    draw = black,
    text = black,
    minimum width = 0.5cm,
    minimum height = 0.5cm] (thetatilde) at (1.5*\layerdist,-8*\nodedist){$\Tilde{\theta}$};
    \draw[signal] (plus) -- (thetatilde);
    
    
    \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:$p_x$}] 
            (Ib1) at ($(0,-1.25*\nodedist) + (0, -8.5*\nodedist)$) {$\gamma( p_x)$}; 
    \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:$ p_y$}] 
            (Ib2) at ($(0,-2.75*\nodedist) + (0, -8.5*\nodedist)$) {$\gamma (p_y)$}; 
    % \foreach \y in {1,2}
    %     \node[inputnode, pin={[pin edge={latex-}, pin distance=\pindist]left:Input \y}] 
    %         (I\y) at (0,-\y*\nodedist) {$p_x$};  
    
    \foreach \y in {1,...,4}
        \node[hiddennode] 
            (Hb\y) at ($(\layerdist,-\y*\nodedist) +(0, 0.5*\nodedist) + (0, -8.5*\nodedist)$) {};
    \foreach \y in {1,...,4}
        \node[hiddennode] 
            (Bb\y) at ($(2*\layerdist,-\y*\nodedist) +(0, 0.5*\nodedist)+ (0, -8.5*\nodedist)$) {};
            
    \node[netnode,fill=red]
            (Ob1) at ($(3*\layerdist,-1*\nodedist)+ (0, -8.5*\nodedist)$) {$R$};
    \node[netnode,fill=green]
            (Ob2) at ($(3*\layerdist,-2*\nodedist)+ (0, -8.5*\nodedist)$) {$G$};
    \node[netnode,fill=blue]
            (Ob3) at ($(3*\layerdist,-3*\nodedist)+ (0, -8.5*\nodedist)$) {$B$};

    
    \foreach \dest in {1,...,4}
        \foreach \source in {1,...,2}
            \draw[signal] (Ib\source) -- (Hb\dest);
    \foreach \dest in {1,...,4}
        \foreach \source in {1,...,4}
            \draw[signal] (Hb\source) -- (Bb\dest);
    \foreach \dest in {1,...,3}
        \foreach \source in {1,...,4}
            \draw[signal] (Bb\source) edge (Ob\dest);
     \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 2.5*\nodedist] (rb1) at (0.5*\layerdist,-10.5*\nodedist) {};
    
    \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 3.5*\nodedist] (rb2) at (1.5*\layerdist,-10.5*\nodedist) {};
    
    \node[rectangle,
    draw = white,
    text = black,
    fill = yellow!100!black,
    minimum width = 0.5cm,
    opacity = 0.5,
    minimum height = 3*\nodedist] (rb3) at (2.5*\layerdist,-10.5*\nodedist) {};
    \foreach \source in {1,3}
        \draw[signal] (thetatilde) -| (rb\source) ;
    \draw[signal] (thetatilde) -- (rb2); 
    
    
    %bitstream
    \coordinate (bitstream) at ($(3.7*\layerdist,-6.15*\nodedist)$);
    \draw[draw=black] (3.5*\layerdist,-6.3*\nodedist) rectangle ++(0.2,0.2);
    \draw[draw=black, fill=black] ($(3.57*\layerdist,-6.3*\nodedist)$) rectangle ++(0.2,0.2);
    \draw[draw=black, fill=black] ($(3.64*\layerdist,-6.3*\nodedist)$) rectangle ++(0.2,0.2);
    \draw[draw=black, fill=white] ($(3.71*\layerdist,-6.3*\nodedist)$) rectangle ++(0.2,0.2);
    \draw[draw=black, fill=black] ($(3.78*\layerdist,-6.3*\nodedist)$) rectangle ++(0.2,0.2);
    \draw[draw=black, fill=white] ($(3.85*\layerdist,-6.3*\nodedist)$) rectangle ++(0.2,0.2);
    
    \draw[signal] (bitstream) |- (decompress) ;
    \draw[signal] (compress) -| (bitstream);
    % \node[annot, above=4pt of H1] (hl) {Hidden layer};
    % \node[annot] at (I1 |- hl) {Input layer};
    % \node[annot] at (O1 |- hl) {Output layer};
\end{tikzpicture}

==> sections/plots.tex <==
\begin{document}

\usepackage{tikz}
\begin{figure*}
	\setlength{\linewidth}{\textwidth}
	\setlength{\hsize}{\textwidth}
% 	\vspace{-9mm}
	\centering
	\renewcommand{\tabcolsep}{0.05pt}
	\renewcommand{\arraystretch}{0.1}
	\begin{tabular}{ccccc}	
	    \footnotesize original & 
		\footnotesize JPEG & 
		\footnotesize JPEG2000 &
		\footnotesize Ours (Meta-learned)  \\	
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.8cm, connect spies}]
			\node {\includegraphics[ width=0.24\linewidth]{img/img_comp/kodim21.png}};
			\spy on (-1.2, 0.2) in node [right] at (-2, -2.1);%(1.6, 0.7);
		\end{tikzpicture} &			
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.8cm, connect spies}]
		 
			\node[label={[font=\footnotesize, xshift=0.7cm, yshift=-4cm, align=center] $0.1720$ bpp\\ $20.67$ dB} ] {\includegraphics[width=0.24\linewidth]{img/img_comp/kodim21_01.jpg}};
			\spy  on (-1.2, 0.2) in node [right] at (-2, -2.1);
		\end{tikzpicture} &			
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.8cm, connect spies}]
			\node[label={[font=\footnotesize, xshift=0.7cm, yshift=-4cm, align=center] $0.0835$ bpp\\ $24.43$ dB} ] {\includegraphics[width=0.24\linewidth]{img/img_comp/kodim21_jpeg2000_open_Q287.png}};
			\spy  on (-1.2, 0.2) in node [right] at (-2, -2.1);
		\end{tikzpicture} &
		% chair
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.8cm, connect spies}]
			\node[label={[font=\footnotesize, xshift=0.7cm, yshift=-4cm, align=center] $0.0829$ bpp\\ $24.43$ dB} ] {\includegraphics[width=0.24\linewidth]{img/img_comp/modelv3_bw7_adaround_iter_1000_adaround_reg_0.0001_retrain_epochs300_retrain_lr1e-06_bpp0.08296712239583333_psnr24.43883332554804.png}};
			\spy on (-1.2, 0.2) in node [right] at (-2, -2.1);
		\end{tikzpicture}
	\end{tabular}

\label{fig:imagecomparisonkodak}
\end{figure*}
\begin{figure*}
    %\setlength{\linewidth}{\textwidth}
    \setlength{\hsize}{\linewidth}
	\centering
	\renewcommand{\tabcolsep}{0.0pt}
	\renewcommand{\arraystretch}{0.2}
	\begin{tabular}{cccc}	
	    \footnotesize original & 
		\footnotesize JPEG & 
		\footnotesize JPEG2000 &
		\footnotesize Ours (Meta-learned)  \\	
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.5cm, connect spies}]
			\node {\includegraphics[ width=0.22\linewidth]{img/img_comp/189091.png}};
			\spy on (-0.35, -0.2) in node [right] at (-0.8, -2);%(1.6, 0.7);
		\end{tikzpicture} &			
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.5cm, connect spies}]
			\node {\includegraphics[width=0.22\linewidth]{img/img_comp/189091_13.jpg}};
			\spy  on (-0.35, -0.2) in node [right] at (-0.8, -2);
		\end{tikzpicture} &			
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.5cm, connect spies}]
			\node {\includegraphics[width=0.22\linewidth]{img/img_comp/189091_jpeg2000_open_Q47.png}};
			\spy  on (-0.35, -0.2) in node [right] at (-0.8, -2);
		\end{tikzpicture} &
		% chair
		\begin{tikzpicture}[spy using outlines={circle,magenta,magnification=2,size=1.5cm, connect spies}]
			\node {\includegraphics[width=0.22\linewidth]{img/img_comp/modelv3_bw7_adaround_iter_1000_adaround_reg_0.0001_retrain_epochs300_retrain_lr1e-06_bpp0.5084011957530151_psnr32.53507601434217.png}};
			\spy on (-0.35, -0.2) in node [right] at (-0.8, -2);
		\end{tikzpicture} &			\\
	%	\vspace{-5mm}
		\footnotesize & 
		\footnotesize $0.526$ bpp & 
		\footnotesize $0.514$ bpp &
		\footnotesize $0.508$ bpp  \\
		\footnotesize & 
		\footnotesize $28.58$ dB & 
		\footnotesize  $31.68$ dB &
		\footnotesize  $32.56$ dB \\		
	\end{tabular}
% 	\vspace{1mm}

\label{fig:imagecomparisonceleb}
\end{figure*}
\end{document}
